Modeling Urban Population Dynamics and City-to-City Migration

Migration plays a crucial role in urban growth. Over time, individuals opting to relocate led to vast metropolises like London and Paris during the Industrial Revolution, Shanghai and Karachi during the last decades and thousands of smaller settlements. Here, we analyze the impact that migration has on population redistribution. We use a model of city-to-city migration as a process that occurs within a network, where the nodes represent cities, and the edges correspond to the flux of individuals. We analyze metrics characterizing the urban distribution and show how a slight preference for some destinations might result in the observed distribution of the population.

==> Notes.tex <==
Los emails de Diego

Please note that overlaps among the chapters should be avoided. Urban hierarchies will probably to some extend by addressed by chapter 16. City size distrubutions represent the content of chapter 9. City growth is in chapter 10.

Your chapter should really focus on the flow (of people) between cities.
I noticed that Rafaels chapter on gravity models (15.) comes after yours (14.). So it might make sense to swap them.


The idea is to cover flows on regional scale, ie between cities.
It should/could include gravitational approaches, radiation model,
https://www.nature.com/articles/s41586-020-2900-x
https://www.nature.com/articles/s41467-020-18205-1
and other sources that need to be identified.


----
El abstract que escribió Filippo.
----
Urban population flows
author: Filippo Simini (confirmed)
Various types of interactions between geographic locations can be represented as spatial flows, such as mobility flows (number of commuters per day or migrants per year), commodity flows (number of parcels delivered per week), and communication flows (number of calls per unit time). Mathematical models to estimate population and mobility flows have important applications, including transportation, urban planning, and epidemic modeling. Traffic congestion, domestic migration, and the spread of infectious diseases are processes in which the presence of mobility flows induces a net change of the spatial distribution of some quantity of interest (vehicles, population, pathogens). The ability to accurately describe the dynamics of these processes depends on our understanding of the characteristics of the underlying spatial flows. This chapter offers an overview of the state-of-the art models to describe spatial interactions, presenting their fundamental assumptions, highlighting the similarities and differences of the various approaches and concludes with a discussion on the latest developments and open challenges in this research area
-----
propuesta
1 - hablar de migración, de los modelos y de sus posibles datos
2 - hablar de las implicaciones de migración en cuanto a la población de ciudades
3 - generar un ejemplito en una markov chain con 5 nodos
4 - utilizar un ejemplo de Madagascar (por ser una isla) con más nodos y analizar el impacto a largo plazo. 
-----




